Variants in managing supply chains on distributed ledgers

Smart contracts show a high potential for ensuring that Supply Chain Management strategies make a qualitative leap toward higher levels of optimality, not only in terms of efficiency and profitability but also in the aggregation of skills aimed at creating the best products and services to bring to the market. In this article, we illustrate an architecture that employs smart contracts to implement various algorithmic versions of the Income Sharing principle between companies participating in a supply chain. We implement our approach on Hyperledger Fabric, the most widespread platform for private and consortium distributed ledgers, and discuss its suitability to our purposes by comparing this design choice with the alternative given by public blockchains, with particular attention to Ethereum.

==> architecture.tex <==
The overall architecture presents three main subsystems (Typescript projects):
\texttt{SupplyChain} realises all aspects of the smart contract,
\texttt{API} provides a collection of APIs to activate transactions, and \texttt{SCWebApp} supports user interaction.

The typical form of the behaviours supported by the architecture starts with the Web app collecting data and passing them to the business logic APIs via some GET or POST HTTP requests, depending on the transaction to execute. The business logic component then uses standard protocols to connect to the ledger and have some transaction executed in it.

Only agents whose credentials are stored (in a "wallet") 
%
%in the application 
%
can have transactions executed.
%
%on the ledger. 
%
Indeed, with every request to an API, a check is performed to retrieve the agent's certificate. 
If it exists, then a \texttt{Gateway} object is instantiated, to connect to the ledger. 
The object has methods to select the contract at hand, to identify the desired transaction, and to submit it. 

In particular, the method \texttt{submitTransaction} will alter the ledger state by recording the transaction in it, while the method \texttt{evalTransaction} just queries the current state.

As a result is obtained, the connection is closed and a JSON object is created of the form $\{\mbox{\texttt{state}},\mbox{\texttt{message}},\mbox{\texttt{body}}\}$, where \texttt{state} is a HTTP-like code indicating the outcome of the request (200 for \texttt{OK}, 500 for \texttt{exception}, 400+ for \texttt{malformed}, for \texttt{not found}, etc.), \texttt{message} is some human-readable informative string and \texttt{body} encodes the actual response (possibly none if the request failed). 

On the ledger side, the functions take the input, parse and convert it if necessary, 
%
%(as the \texttt{submitTransaction} and \texttt{evalTransaction} methods can only pass strings, the numerical parameters in the algorithm must be converted), 
%
and execute the transactions
%
%with the converted values.

Figure~\ref{fig:overall} describes the communication structure among components (and the used protocols) supporting the management of a request to the Web application resulting in a transaction to be executed on the ledger, according to the contract, as established
once the \texttt{SupplyChain} smart contract has been installed on the \texttt{Hyperledger}, 
a \texttt{Gateway} has been instantiated to manage communication towards it and the \texttt{Wallet} component to manage credentials is active\footnote{The Wallet component might be an encrypted file or a separate database.}. 
%
%Labels of arrows indicate the communication protocol.

\begin{figure}[htb]
    \centering
    \includegraphics[width=\linewidth]{figures/Overall.png}
    \caption{The main components and communication structure.}
    \label{fig:overall}
\end{figure}

%Figure~\ref{fig:enrolment} summarises 
%
The 
%
%sequence of 
%
activities leading to its construction 
%
%of such a communication structure 
%
can be summarised as follows.
%
%, where \texttt{DeploySC} is a complex activity performed only once 
%
First, the contract is deployed according to protocols in Fabric, 
possibly using existing scripts\footnote{We do not go into technical details here, see https://hyperledger-fabric.readthedocs.io/en/release-2.2/deploy\_chaincode.html\#typescript.}. 
%
%The activities in the loop are performed with each request of a transaction. 
%
Then, for each transaction request, a connection profile (CP) is created, and the certificate is checked on the wallet associated with it.
%
%Note that we do not specify a final node for the activity, since, even when the transactions corresponding to the distributions of %revenues have been performed, the contract might remain active for replying to queries on its execution. 
%Inside the loop, \texttt{SetUpGateway}.
%
After that, setting up the gateway requires three steps: 
\begin{inparaenum}[(1)]
\item initialise it with the CP;
\item obtain a connection for the channel to be used, invoking 
%
%(via the \texttt{getNetwork(channelName)} method)
%
\texttt{getNetwork(chName)}; and 
\item obtain reference to the 
%
%deployed 
%
contract code, 
%
%passing the identifier of the contract 
%(i.e., invoking \texttt{getRequestById(reqId)}).
%
via \texttt{getReqById(reqId)}).
\end{inparaenum}
%
After that, the transaction is applied, invoking the corresponding function and passing the response back to the Web app, and the gateway is closed. Figure~\ref{fig:enrolment} summarises the activities described above.

\begin{figure}[htb]
    \centering
    \includegraphics[width=\linewidth]{figures/enrolment.png}
    \caption{Activities for managing interaction with a deployed contract.}
    \label{fig:enrolment}
\end{figure}

% Figure~\ref{fig:overallFlow} shows a generic message flow for managing a user request (from either an originator or a supplier \emph{participant}). %Responses to requests authorised

% \begin{figure*}[htb]
%     \centering
%     \includegraphics[width=0.6\linewidth]{figures/OverallFlow.png}
%     \caption{The generic message flow to manage transactions.}
%     \label{fig:overallFlow}
% \end{figure*}

==> smart.tex <==
We first sketch how the information provided by originator and suppliers, conceptually maintained in a collection of matrices, is represented in the data structures of the 
%
\texttt{SupplyChain} module managing the smart contract, in the 
%
Node.js/TypeScript implementation realised in Fabric.

Information from the originator is used to instantiate the fundamental data structure of the implementation, a \texttt{Request} object, unique to the supply chain. 
Such an object implements the matrices in the form of an array of \texttt{TreeLevel} objects, where each instance of \texttt{TreeLevel} maintains a number identifying the level, and an array of \texttt{Resource} objects. 

For each type of resource $k$ (at level $i$), the parameter $BOM_{ik}$ and a value $g$ describing the overall share of revenue for that type
%
%, as defined by the negotiation, 
%
are used (in an interaction not shown here) to initialise the corresponding instance of \texttt{Resource}. 
The latter
also maintains 
%
%a \texttt{supplyList}, i.e., 
%
an array of \texttt{Supply} objects, describing the commitments of specific suppliers to provide a certain number of resources, through the parameters described in Section \ref{sec:algorithm}.

Figure~\ref{fig:smartContract} provides a conceptual overview of the resulting data structures in the \texttt{SupplyChain} module. 
We follow here the TypeScript implementation in the definition of types, thus using \texttt{number} for floating point values.
For legibility, we show only the features with which objects are instantiated. 
The remaining features model parameters which are either interactively entered by the supplier, i.e., $cf_{ikm},cv_{ikm},qp_{ikm},tp_{ikm},g_{ik}$, or calculated during the execution of the algorithm, e.g., $f_{ikm}$ or $c^{min}_{ik}$. 

\begin{figure}[htb]
    \centering
    \includegraphics[width=\linewidth]{figures/WebApp.png}
    \caption{A partial view of the data structures for the Supply Chain.} 
    %
    %smart contract. Only members set at instantiation time are shown.
    \label{fig:smartContract}
\end{figure}

Figure~\ref{fig:createRequest} shows the interaction for an originator to create a request, while Figure~\ref{fig:createSupply} shows the interaction for a supplier agent to define the form of participation in the supply chain.

\begin{figure}[htb]
    \centering
    \includegraphics[width=\linewidth]{figures/createRequest.png}
    \caption{The interface for creating a request}
    \label{fig:createRequest}
\end{figure}

\begin{figure}[htb]
    \centering
    \includegraphics[width=\linewidth]{figures/createSupply.png}
    \caption{The interface for detailing a supplier's commitment.}
    \label{fig:createSupply}
\end{figure}

The steps of the algorithm are implemented as a collection of functions, one for each step, invoked, in order, through a public asynchronous function \texttt{RevenueSharing}, contained in the \texttt{SupplyChain} module. 
Each step receives the relevant \texttt{Request} object as input and is typed as \texttt{void}, except for the invocation of step 5, which returns an array of $(supplier,revenue)$ pairs. 
Each of these functions produces a suitable value for some feature in the relevant \texttt{Resource} 
(e.g., $c^{min}_{ik}$) or \texttt{Supplier} objects (e,g,, $f_{ikm}$).

The 
%
%\texttt{SupplyChain} 
%
module also contains a collection of functions for the transactions available. 
Besides the \texttt{RevenueSharing} transition starting the algorithm, 
%
%through an asynchronous call to the \texttt{RevenueSharing} function, 
%
we have:
\begin{itemize}
    \item \texttt{createRequest(params)} instantiates on the ledger a new \texttt{Request} object, initialised with the passed parameters and with a unique ID;
    \item \texttt{addLevel(reqID)} creates a new \texttt{TreeLevel} in the identified \texttt{Request} object;
    \item \texttt{existResource(reqID,level,resNm)} checks the existence of a resource at a certain level for a request;
    \item \texttt{createResource(reqID,level,params)} instantiates a \texttt{Resource} object for the identified request, at the required level; 
    \item \texttt{getReqById(reqID)} retrieves a \texttt{Request} object, for further manipulation, while \texttt{getReqByOrig} \texttt{(origID)} retrieves all the requests from an originator;
    \item \texttt{createSupply(reqID,resourceName,level,} \texttt{supplierID,params)} creates an instance of \texttt{Supply} describing the contribution of that supplier for a certain resource at a certain level, characterised by the provided parameters, and inserts it in the \texttt{supplyList} associated with the resource at that level.
\end{itemize}

Figure~\ref{fig:detailsWithRevenues} shows the page representing to participants the final situation after revenues have been shared.

\begin{figure*}[htb]
    \centering
    \includegraphics[width=.96\linewidth]{figures/detailsWithRevenues.png}
    \caption{A summary presentation of the supply chain with revenue sharing.}
    \label{fig:detailsWithRevenues}
\end{figure*}

